Graph-Structured Speculative Decoding

Speculative decoding has emerged as a promising technique to accelerate the inference of Large Language Models (LLMs) by employing a small language model to draft a hypothesis sequence, which is then validated by the LLM. The effectiveness of this approach heavily relies on the balance between performance and efficiency of the draft model. In our research, we focus on enhancing the proportion of draft tokens that are accepted to the final output by generating multiple hypotheses instead of just one. This allows the LLM more options to choose from and select the longest sequence that meets its standards. Our analysis reveals that hypotheses produced by the draft model share many common token sequences, suggesting a potential for optimizing computation. Leveraging this observation, we introduce an innovative approach utilizing a directed acyclic graph (DAG) to manage the drafted hypotheses. This structure enables us to efficiently predict and merge recurring token sequences, vastly reducing the computational demands of the draft model. We term this approach Graph-structured Speculative Decoding (GSD). We apply GSD across a range of LLMs, including a 70-billion parameter LLaMA-2 model, and observe a remarkable speedup of 1.73$\times$ to 1.96$\times$, significantly surpassing standard speculative decoding.

==> tables/attention.tex <==
\begin{table*}[t]
\begin{center}
\setlength{\tabcolsep}{1.2mm}{
\scalebox{1}{\begin{tabular}{lllrlrl}
\toprule
Methods & Attention Regions & Is causal? & \multicolumn{2}{c}{LLAMA-65B} & \multicolumn{2}{c}{LLAMA-30B}  \\
\midrule
\textsc{Random Guess} & - & - & $43.06$& & $43.06$ \\
\midrule
\textsc{Regular ICL} & \ding{172}+\ding{173} & Yes & $59.83$ & ($+16.77$) & $52.71$ & ($+9.65$)\\
\textsc{Full Attn.} (v1) & \ding{172}+\ding{173}+\ding{177} & No  & 45.15 & ($+2.09$) & 47.84 & ($+4.78$) \\
\textsc{Full Attn.} (v2) & \ding{172}+\ding{173}+\ding{177}+\ding{178} & No & $44.32$ & ($+1.26$) & $47.36$ & ($+4.30$) \\
\midrule
\textsc{Rd} & \ding{172}+\ding{173}+\ding{174}+\ding{175}+\ding{176} & Yes & $60.18$ & ($+17.12$) & $54.02$ & ($+10.96$)\\
\textsc{RdSca} w/o \texttt{<SOS>} & \ding{172}+\ding{173}+\ding{174} & Yes & $32.20$ & ($-10.86$) & $12.96$ & ($-30.10$)\\
\midrule
\textsc{RdSca}  & \ding{172}+\ding{173}+\ding{174}+\ding{175} & Yes & $64.96$& ($+\textbf{21.90}$) & 56.55 & ($+\textbf{13.49}$)\\
% \midrule
% & \ding{172}+\ding{173}+\ding{177}+\ding{178}+\ding{179} \\
\bottomrule
\end{tabular}}}
\end{center}
\caption{Ablations on causal attention customization. We report the averaging performance on all tasks. We implement two versions of the \textsc{Full Attn.}, which differ in whether including left-to-right attention of the query.}
\label{tab:attn}
\vspace{-1mm}
\end{table*}



% \begin{figure*}[ht]
%   \centering
%   \begin{subfigure}[b]{0.3\linewidth}
%       \includegraphics[width=0.2\textwidth]{figures/attention.pdf}
%       \caption{Illustration of attention regions.}
%       \label{fig:attn}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.7\linewidth}
%       \centering
%       \scalebox{0.8}{\begin{tabular}{lllrlrl}
%         \toprule
%         Methods & Attention Regions  & \multicolumn{2}{c}{LLAMA-65B} & \multicolumn{2}{c}{LLAMA-30B}  \\
%         \midrule
%         \textsc{Random Guess} & - & $43.06$& & $43.06$ \\
%         \midrule
%         \textsc{Regular ICL} & \ding{172}+\ding{173}  & $57.32$ & ($+14.26$) & $50.45$ & ($+7.39$)\\
%         \textsc{Full Attn.} (v1) & \ding{172}+\ding{173}+\ding{177}  & 45.15 & ($+2.09$) & 47.84 & ($+4.78$) \\
%         \textsc{Full Attn.} (v2) & \ding{172}+\ding{173}+\ding{177}+\ding{178}& $44.32$ & ($+1.26$) & $47.36$ & ($+4.30$) \\
%         \midrule
%         \textsc{Rd} & \ding{172}+\ding{173}+\ding{174}+\ding{175}+\ding{176}  & $57.82$ & ($+14.76$) & $51.71$ & ($+8.65$)\\
%         \textsc{RdSca} w/o \texttt{<SOS>} & \ding{172}+\ding{173}+\ding{174}  & $32.20$ & ($-10.86$) & $12.96$ & ($-30.10$)\\
%         \midrule
%         \textsc{RdSca}  & \ding{172}+\ding{173}+\ding{174}+\ding{175} & $63.34$& ($+\textbf{20.28}$) & 54.70 & ($+\textbf{11.64}$)\\
%         % \midrule
%         % & \ding{172}+\ding{173}+\ding{177}+\ding{178}+\ding{179} \\
%         \bottomrule
%         \end{tabular}}
%   \end{subfigure}
  
% \end{figure*}


% Illustration of the attention mask, which we divide into multiple regions and label with numbers. The specific meanings are as follows: \ding{172} query-to-demonstrations attention; \ding{173} inter-demonstrations right-to-left attention; \ding{174} inter-demonstrations(repeat) right-to-left attention; \ding{175} attention to the start-of-sentence token; \ding{176} attention to redundant context; \ding{177} inter-demonstrations left-to-right attention;\ding{178} demonstrations-to-query attention;\ding{179} other left-to-right attention.

==> tables/instruction.tex <==
\begin{table}[h]
\begin{center}
\setlength{\tabcolsep}{1.2mm}{
\scalebox{0.8}{\begin{tabular}{lllll}
\toprule
Methods & 65B & 30B & 13B & 7B \\
\midrule
\textit{with instruction} \\
\textsc{Regular ICL} &  69.87 & 63.1 & 57.86 & 59.17 \\
\textsc{Rd} &  71.28 & 67.34 & 59.2 & 60.22 \\
\textsc{RdSca} &  74.27 & 68.73 & 61.11 & 59.73 \\
\midrule
\textit{without instruction} \\

\bottomrule
\end{tabular}}}
\end{center}
\caption{Full evaluation results on CB}
\vspace{-1mm}
\end{table}

==> tables/mmlu.tex <==
\begin{table}[h]
    \centering
      \scalebox{1}{\begin{tabular}{lll}
        \toprule
         & \textsc{Regular ICL} & \textsc{RdSca}  \\
        \toprule
        humanities & 65.99 & 68.44\\
        STEM & 51.84 & 51.57\\
        social sciences & 72.29 & 73.60\\
        other & 63.34 & 64.65\\ \midrule
        average  & 62.20 & 63.66\\
        \bottomrule
      \end{tabular}}
      \caption{LLAMA-65B 4-shot ICL results on MMLU.}
      \label{mmlu}
\end{table}

==> tables/window.tex <==
% \begin{figure}[ht]
%   \centering
%   \begin{subfigure}[c]{\linewidth}
%       \includegraphics[width=1.\linewidth]{figures/window.pdf}
%       \label{fig:res}
%   \end{subfigure}
%   \begin{subfigure}[c]{\linewidth}
%       \centering
%       \begin{tabular}{lcccc}
%         \toprule
%         Window & n-shots & LLAMA-65B & LLAMA-30B \\
%         \toprule
%         regular & 0-1-2-3-4 & 69.87 & 63.10 \\
%         \midrule
%         W=1 & 0-0-0-0-4 & 60.83 & 52.78 \\
%         W=2 & 1-1-1-1-4 & 71.33 & 60.83 \\
%         W=3 & 2-2-2-2-4 & 74.01 & 65.70 \\
%         W=4 & 3-3-3-3-4 & 74.27 & 68.73 \\
%         \bottomrule
%       \end{tabular}
%   \end{subfigure}
%   \caption{Visualization of attention masks for different window sizes where $K=4$.}
% \end{figure}

\begin{figure}[th]
  \centering
  \includegraphics[width=1.\linewidth]{figures/window.pdf}
  \caption{Visualization of attention masks for different window sizes.}
  \label{fig:window}
\end{figure}
\begin{table}[h]
    \centering
    \centering
      \scalebox{0.85}{\begin{tabular}{lcccc}
        \toprule
        Window & n-shots & LLAMA-65B & LLAMA-30B \\
        \toprule
        \textsc{Regular} & 0-1-2-3-4 & $69.87$ & $63.10$ \\
        \midrule
        W=1 & 0-0-0-0-4 & $60.83$ & $52.78$ \\
        W=2 & 1-1-1-1-4 & $71.33$ & $60.83$ \\
        W=3 & 2-2-2-2-4 & $74.01$ & $65.70$ \\
        W=4 & 3-3-3-3-4 & $74.27$ & $68.73$ \\
        \midrule
        W=4 & 3-3-3-3-3 & $70.99$ & $64.44$ \\
        \bottomrule
      \end{tabular}}
    \caption{Average performance on all tasks for different attention window sizes. We also report the number of demonstrations contained in the context of each demonstration. For example, "0-1-2-3-4" means that, for regular ICL, the first demonstration has no context, the second sees one demonstration, the third sees two, and so on. In this experiment, we use \textsc{KATE} to retrieve demonstrations instead of random-selected ones. In this way, we save computational resources because there is no need to run experiments over different random seeds.}
    \label{tab:window}
\end{table}
      

